Dynamical evolution of V-type photometric candidates in the outer Main-belt

V-type asteroids, characterized by two absorption bands at 1.0 and 2.0 $\mu m$, are usually thought to be portions of the crust of differentiated or partially differentiated bodies. Most V-type asteroids are found in the inner main belt and are thought to be current or past members of the Vesta dynamical family. Recently, several V-type photometric candidates have been identified in the central and outer main belt. While the dynamical evolution of V-type photometric candidates in the central main belt has been recently investigated, less attention has been given to the orbital evolution of basaltic material in the outer main belt as a whole. Here we identify known and new V-type photometric candidates in this region, and study their orbital evolution under the effect of gravitational and non-gravitational forces. A scenario in which a minimum of three local sources, possibly associated with the parent bodies of (349) Dembowska, (221) Eos, and (1459) Magnya, could in principle explain the current orbital distribution of V-type photometric candidates in the region.

==> list_diff <==
9a10,11
> \usepackage[normalem]{ulem}
> 
15c17
< \author[M.E. Huaman,V. Carruba, R. C. Domingos]{ M.E. Huaman$^{1}$\thanks{E-mail: mariela@feg.unesp.br}, V. 
---
> \author[M.E. Huaman,V. Carruba, R. C. Domingos]{ M.E. Huaman$^{1}$\thanks{E-mail: mariela@feg.unesp.br}, V.
19c21
< $^{2}$UNESP, Univ. Estadual Paulista, S\~{a}o Jo\~{a}o da Boa Vista, SP, 
---
> $^{2}$UNESP, Univ. Estadual Paulista, S\~{a}o Jo\~{a}o da Boa Vista, SP,
34c36
< {\bf V-type asteroids, characterized by two absorption bands at 1.0 and
---
> \textbf{V-type asteroids, characterized by two absorption bands at 1.0 and
39c41
< V-type photometric candidates have been identified in the central and 
---
> V-type photometric candidates have been identified in the central and
42,43c44,45
< While the dynamical evolution of V-type photometric candidates 
< in the central main belt has been recently investigated, less attention 
---
> While the dynamical evolution of V-type photometric candidates
> in the central main belt has been recently investigated, less attention
46c48
< known and new V-type photometric candidates in this region, and study their 
---
> known and new V-type photometric candidates in this region, and study their
48,50c50,52
< forces.  A scenario in which a minimum of three local sources, possibly 
< associated with the parent bodies of (349) Dembowska, (221) Eos, and (1459) 
< Magnya, could in principle explain the current orbital distribution of V-type 
---
> forces.  A scenario in which a minimum of three local sources, possibly
> associated with the parent bodies of (349) Dembowska, (221) Eos, and (1459)
> Magnya, could in principle explain the current orbital distribution of V-type
55c57
< Minor planets, asteroids: general -- Celestial mechanics.  
---
> Minor planets, asteroids: general -- Celestial mechanics.
63,72c65,74
< Basaltic asteroids are associated with the crust of differentiated 
< body. They are usually associated with a V-type spectrum, 
< characterized by absorptions bands at 1 and 2 $\mu$ m. 
< The majority of basaltic asteroids are found in the inner 
< main belt, although a few have also been observed in the outer 
< main belt.  The first evidence for another possible source of 
< basaltic asteroid in the outer main belt was the asteroid (1459) 
< Magnya discovery by Lazarro et al. (2000). Other autors as 
< Michtchenko et al. (2002) suggested that Magnya is a fragment 
< from a differentiated parent body that broke up in 
---
> Basaltic asteroids are associated with the crust of differentiated
> body. They are usually associated with a V-type spectrum,
> characterized by absorptions bands at 1 and 2 $\mu$ m.
> The majority of basaltic asteroids are found in the inner
> main belt, although a few have also been observed in the outer
> main belt.  The first evidence for another possible source of
> basaltic asteroid in the outer main belt was the asteroid (1459)
> Magnya discovery by Lazarro et al. (2000). Other autors as
> Michtchenko et al. (2002) suggested that Magnya is a fragment
> from a differentiated parent body that broke up in
75,76c77,78
< The discovery and analysis of basaltic asteroids independent of Vesta 
< can provide insights into the early history of solar system formation 
---
> The discovery and analysis of basaltic asteroids independent of Vesta
> can provide insights into the early history of solar system formation
78,79c80,81
< bodies that were scattered into the central and outer main belt 
< is not well understood or constrained by previous models, 
---
> bodies that were scattered into the central and outer main belt
> is not well understood or constrained by previous models,
82c84
< to the formation of the Veneneia crater on Vesta, Milani et al. 2013), 
---
> to the formation of the Veneneia crater on Vesta, Milani et al. 2013),
84c86
< bodies other than Vesta into the central and outer main belt, 
---
> bodies other than Vesta into the central and outer main belt,
90,95c92,97
< This work, {\bf that is the continuation of an analogous study
< performed in the central main belt (Carruba et al. 2014b),} is so 
< divided: in Section 2 we revise 
< spectral taxonomy of asteroids in the outer main belt 
< and identify possible V-type 
< photometric candidates. In Section 3 we define groups 
---
> This work, \textbf{that is the continuation of an analogous study
> performed in the central main belt (Carruba et al. 2014b),} is so
> divided: in Section 2 we revise
> spectral taxonomy of asteroids in the outer main belt
> and identify possible V-type
> photometric candidates. In Section 3 we define groups
98c100
< Section 5 is dedicated to the Yarkovsky orbital evolution, with a 
---
> Section 5 is dedicated to the Yarkovsky orbital evolution, with a
100c102
< Finally, we present our conclusions in Section {\bf 6}.
---
> Finally, we present our conclusions in Section \textbf{6}.
109,110c111,112
< and ${z}'-{i}'$ colors. In that article the authors used the photometric 
< data obtained in the five filters $ u', g', r', i'$, and $z'$, from 0.3 
---
> and ${z}'-{i}'$ colors. In that article the authors used the photometric
> data obtained in the five filters $ u', g', r', i'$, and $z'$, from 0.3
112c114
< These data were then used to determine if an asteroid belonged to a given 
---
> These data were then used to determine if an asteroid belonged to a given
115c117
< details on their classification method, we refer the reader to the 
---
> details on their classification method, we refer the reader to the
122,125c124,127
< classified as V-types (1459 Magnya, Lazzaro et al. (2000), 7472 Kumakiri, 
< Duffard and Roig (2009), 10537 1991 RY16 Moskovitz et al. (2008), 14390 
< 1990 QP19, De Sanctis (2011a,b), 105041 2000 K041, De Sanctis et al. 
< (2011a,b)).  {\bf Six objects (11465, 55270, 91159, 92182, 177904, 
---
> classified as V-types (1459 Magnya, Lazzaro et al. (2000), 7472 Kumakiri,
> Duffard and Roig (2009), 10537 1991 RY16 Moskovitz et al. (2008), 14390
> 1990 QP19, De Sanctis (2011a,b), 105041 2000 K041, De Sanctis et al.
> (2011a,b)).  \textbf{Six objects (11465, 55270, 91159, 92182, 177904,
127,132c129,134
< one (34698 2001 OD22, also listed in the 
< WISE albedo catalog\footnote{Initial results from the Wide-field 
< Infrared Survey Explorer (WISE) (Wright et al. 2010), and the NEOWISE 
< (Mainzer et al. 2011) enhancement 
< to the WISE mission recently allowed to obtain diameters and 
< geometric albedo values for more than 100,000 Main Belt asteroids 
---
> one (34698 2001 OD22, also listed in the
> WISE albedo catalog\footnote{Initial results from the Wide-field
> Infrared Survey Explorer (WISE) (Wright et al. 2010), and the NEOWISE
> (Mainzer et al. 2011) enhancement
> to the WISE mission recently allowed to obtain diameters and
> geometric albedo values for more than 100,000 Main Belt asteroids
135,141c137,143
< V-type asteroid candidate were identified in the past by 
< Carvano et al. (2010).  These authors used studies on taxonomy 
< of asteroids observed by the Sloan Digital Sky Survey-Moving Object 
< Catalog data, fourth (SDSS-MOC4 hereafter), and identified 52 
< V-type photometric candidates in the outer main belt, including 
< objects with QS, SV, and other cases. This database is available 
< on the Planetary Data System (http:sbn.psi.edu/pds/resource/sdsstax.html, 
---
> V-type asteroid candidate were identified in the past by
> Carvano et al. (2010).  These authors used studies on taxonomy
> of asteroids observed by the Sloan Digital Sky Survey-Moving Object
> Catalog data, fourth (SDSS-MOC4 hereafter), and identified 52
> V-type photometric candidates in the outer main belt, including
> objects with QS, SV, and other cases. This database is available
> on the Planetary Data System (http:sbn.psi.edu/pds/resource/sdsstax.html,
144,146c146,148
< With respect to this database, we selected all asteroids that were 
< V-type photometric candidates (including object with QS, SV and 
< other cases) and identified according to the HORIZONS System of the 
---
> With respect to this database, we selected all asteroids that were
> V-type photometric candidates (including object with QS, SV and
> other cases) and identified according to the HORIZONS System of the
148,149c150,151
< V-type asteroids, we encountered 25 V-type candidates that are pure V 
< (excluding QS and SV cases) and have proper elements as 
---
> V-type asteroids, we encountered 25 V-type candidates that are pure V
> (excluding QS and SV cases) and have proper elements as
151,153c153,155
< identified in this work {\bf and in Carruba et al. (2014b)}, and 
< the five confimed V-type objects, 
< we have a total of 37 asteroids that are possible or confirmed V-types 
---
> identified in this work \textbf{and in Carruba et al. (2014b)}, and
> the five confimed V-type objects,
> we have a total of 37 asteroids that are possible or confirmed V-types
157c159
< \begin{figure*}
---
> \begin{figure}
166,169c168,171
< \caption{Panel A: Proper semi-major axis versus 
< eccentricity of the V-type candidates identified using SDSS-MOC4 data 
< in the outer main belt. Panel B: Semi-major 
< axis versus sine of proper incliation of the V-type candidates.
---
> \caption{Panel A: Proper semi-major axis versus
> eccentricity of the V-type candidates identified using SDSS-MOC4 data
> in the outer main belt. Panel B: Semi-major
> axis versus sine of proper inclination of the V-type candidates.
175c177
< \end{figure*}
---
> \end{figure}
179,180c181,182
< and $(a,sin(i))$ (panel B) projections of the proper elements of 
< all candidates (black dots), the pure V-type candidates 
---
> and $(a,sin(i))$ (panel B) projections of the proper elements of
> all candidates (black dots), the pure V-type candidates
182,185c184,187
< (red full dots). Vertical lines represent the location of 
< the main local mean-motion resonances, blue lines show 
< the positions of the center of secular resonances, computed 
< using the analytical theory 
---
> (red full dots). Vertical lines represent the location of
> the main local mean-motion resonances, blue lines show
> the positions of the center of secular resonances, computed
> using the analytical theory
189c191
< values of angles and eccentricity of (31) Euphrosyne, the asteroid with the 
---
> values of angles and eccentricity of (31) Euphrosyne, the asteroid with the
192,193c194,195
< We can observe in Fig.~\ref{fig: V-type_external} 
< three regions of concentrations of V-types candidates in 
---
> We can observe in Fig.~\ref{fig: V-type_external}
> three regions of concentrations of V-types candidates in
195,196c197,198
< and is between the resonances 7J:-3A and 2J:-1A. This region includes 
< the confirmed V-type asteroid (1459) Magnya, with a range values 
---
> and is between the resonances 7J:-3A and 2J:-1A. This region includes
> the confirmed V-type asteroid (1459) Magnya, with a range values
198c200
< A higher concentration near the Eos family is found in the center of the 
---
> A higher concentration near the Eos family is found in the center of the
200c202
< as a possible source of basaltic material in the past, 
---
> as a possible source of basaltic material in the past,
202c204
< with $0.00<sin(i)<0.24$.   Finally, in the region 
---
> with $0.00<sin(i)<0.24$.   Finally, in the region
204c206
< we found some scattered objects that may have passed through 
---
> we found some scattered objects that may have passed through
207,208c209,210
< family, and because of the presence of the Koronis family in the 
< region, another possible source of differentiated objects, 
---
> family, and because of the presence of the Koronis family in the
> region, another possible source of differentiated objects,
218,221c220,223
< Eq.~1), the probability that a number of objects be produced by a Poisson 
< distribution assuming that the expected number of k occurrence 
< in a given interval is given by {\bf Eq.~1 in Carruba et al. 2014b.
< For our purposes we used  for the expected number of occurrences 
---
> Eq.~1), the probability that a number of objects be produced by a Poisson
> distribution assuming that the expected number of k occurrence
> in a given interval is given by \textbf{Eq.~1 in Carruba et al. 2014b.
> For our purposes we used  for the expected number of occurrences
223,224c225,226
< the mean values of objects expected in the regions of 
< the Koronis and Eos families, given by Eq.~2 in Carruba et al. 2014b.
---
> the mean values of objects expected in the regions of
> the Koronis and Eos families, given by Eq.~2 in Carruba et al. 2014b.}
226,232c228,234
< We used simple papelelepipedal regions for the areas occupied by the Koronis 
< and Eos families, defined according to the minimum and maximum values in 
< $(a,e,sin(i))$ observed for the halos of these two families in Carruba et 
< al. (2013), defined as $2.828 < a < 2.987, 0.0112 < e < 0.082,  0.0128 
< < sin(i)< 0.058$, and $2.915< a < 3.186, 0.036 < e < 0.108, 0.144 < sin(i) 
< < 0.207$, respectively.  $v_{Tot}$, the total volume occupied by 
< all photometric candidates, was defined as the region between the 
---
> \textbf{We used simple papelelepipedal regions for the areas occupied by the Koronis
> and Eos families, defined according to the minimum and maximum values in
> $(a,e,sin(i))$ observed for the halos of these two families in Carruba et
> al. (2013), defined as $2.828 < a < 2.987, 0.0112 < e < 0.082,  0.0128
> < sin(i)< 0.058$, and $2.915< a < 3.186, 0.036 < e < 0.108, 0.144 < sin(i)
> < 0.207$, respectively.  $v_{Tot}$, the total volume occupied by
> all photometric candidates, was defined as the region between the
234c236
< (i.e., $2.8258 < a < 3.279$ AU), and eccentricity and $sin(i)$ from zero 
---
> (i.e., $2.8258 < a < 3.279$ AU), and eccentricity and $sin(i)$ from zero
236,242c238,244
< 0.2738 and 0.4.  Using Eq.~1 in Carruba et al. (2014b),} we found that the 
< probability that the two asteroids in the Koronis family region, and the 
< six in the Eos paralelepipedal region (four of these objects are not 
< members of the Eos dynamical family) could be explained as fluctuations of a 
< Poissonian distribution are of $ 4.53\cdot 10^{−2}$, and $2.53\cdot 10^{−4}$. 
< Considering that the null hypothesis threshold is equal to 
< $1.0 \cdot 10^{−2})$, while the results for the Koronis region may possibly
---
> 0.2738 and 0.4.  Using Eq.~1 in Carruba et al. (2014b),} we found that the
> probability that the two asteroids in the Koronis family region, and the
> six in the Eos paralelepipedal region (four of these objects are not
> members of the Eos dynamical family) could be explained as fluctuations of a
> Poissonian distribution are of $ 4.53\cdot 10^{−2}$, and $2.53\cdot 10^{−4}$.
> Considering that the null hypothesis threshold is equal to
> $1.0 \cdot 10^{−2}$, while the results for the Koronis region may possibly
244c246
< those for the Eos region seem more robust and may  
---
> those for the Eos region seem more robust and may
247c249
< Since 1-dimensional statistical analysis are somewhat 
---
> Since 1-dimensional statistical analysis are somewhat
249,250c251,252
< the approach of Carruba et al. (2014b), we also perfomed 
< Mardia’s test (Mardia 1970) on multivariate normality 
---
> the approach of Carruba et al. (2014b), we also perfomed
> Mardia’s test (Mardia 1970) on multivariate normality
254,256c256,258
< excludes that V-type photometric candidates follow a tri-variate 
< Gaussian distribution as a whole. In the 
< next section we will further analyze the three orbital regions 
---
> excludes that V-type photometric candidates follow a tri-variate
> Gaussian distribution as a whole. In the
> next section we will further analyze the three orbital regions
266c268
< \begin{figure*}
---
> \begin{figure}
275c277
<    
---
> 
277c279
< in the outer main belt.  Distances with respect to the asteroids 
---
> in the outer main belt.  Distances with respect to the asteroids
281c283
< \end{figure*}
---
> \end{figure}
286c288
< of all photometric V-type candidates in the outer main belt with 
---
> of all photometric V-type candidates in the outer main belt with
288,297c290,299
< (158) Koronis and (349) Dembowska, (221) Eos, and (1459) Magnya.  To 
< determine the distances we used {\bf the} standard
< metrics of Zappal\'a et al. (1995) {\bf (see also Eq.~7 in Carruba et al. 
< 2014b)}. Results are shown in the three panels of Fig.~\ref{fig: velo1}. 
< Asteroids with distances $d$ with respect to (158) Koronis (panel A), 
< (221) Eos (panel B), and (1459) Magnya (panel C) less than 
< $1000~$m/s are rendered as red full dots, those with 
< $1000 < d < 3000~$m/s are shown as yellow full dots, and 
< green full dots identify the objects with $d > 3000~$m/s. 
< The other symbols are the same as in Fig.~\ref{fig: V-type_external}. 
---
> (158) Koronis and (349) Dembowska, (221) Eos, and (1459) Magnya.  To
> determine the distances we used \textbf{the} standard
> metrics of Zappal\'a et al. (1995) \textbf{(see also Eq.~7 in Carruba et al.
> 2014b)}. Results are shown in the three panels of Fig.~\ref{fig: velo1}.
> Asteroids with distances $d$ with respect to (158) Koronis (panel A),
> (221) Eos (panel B), and (1459) Magnya (panel C) less than
> $1000~$m/s are rendered as red full dots, those with
> $1000 < d < 3000~$m/s are shown as yellow full dots, and
> green full dots identify the objects with $d > 3000~$m/s.
> The other symbols are the same as in Fig.~\ref{fig: V-type_external}.
300c302
< objects (11465 and 34698) in the Magnya region, the closest objects to each 
---
> objects (11465 and 34698) in the Magnya region, the closest objects to each
302c304
< region, suggesting that the regions that we proposed in the 
---
> region, suggesting that the regions that we proposed in the
307c309
< candidates with diameter values from the WISE mission (12 objects) 
---
> candidates with diameter values from the WISE mission (12 objects)
309c311
< of Harris and Largeros (2002)  {\bf (see also Eq.~8 in Carruba et al. 
---
> of Harris and Largeros (2002)  \textbf{(see also Eq.~8 in Carruba et al.
311,315c313,317
< of the albedo $p_V$ were 0.040 and 0.392, respectively.  Our results are 
< shown in Fig.~\ref{fig: diameters}, where larger asteroids with 
< $D > 5$ km are shown as red full dots, yellow full dots show the 
< position of the asteroids with $3 < D < 5$~km, and the green dots 
< are associated with smaller bodies. 
---
> of the albedo $p_V$ were 0.040 and 0.392, respectively.  Our results are
> shown in Fig.~\ref{fig: diameters}, where larger asteroids with
> $D > 5$ km are shown as red full dots, yellow full dots show the
> position of the asteroids with $3 < D < 5$~km, and the green dots
> are associated with smaller bodies.
317c319
< To estimate how much mass in the currently known V-type 
---
> \textbf{In order }to estimate how much mass in the currently known V-type
319,321c321,323
< from Carruba et al. (2014b) (Moskovitz et al. 2008), 
< where the bulk density was {\bf assumed equal to $3000~$kg/m$^3$, value typical
< of V-type objects.  For our candidates, we obtained a 
---
> from Carruba et al. (2014b) (Moskovitz et al. 2008),
> where the bulk density was \textbf{ assumed equal to $3000~$kg/m$^3$, value typical
> of V-type objects.  For our candidates, we obtained a
323c325
< of the estimated mass escavated from craters in Vesta $1.3 \cdot 10^{18}$~kg; 
---
> of the estimated mass escavated from craters in Vesta $1.3 \cdot 10^{18}$~kg;
325,327c327,329
< total mass of V-type candidates in the central main belt, but still a 
< very small fraction of the observed basaltic material in the inner main belt.} 
< In the next section we will discuss how V-type photometric candidates 
---
> total mass of V-type candidates in the central main belt, but still a
> very small fraction of the observed basaltic material in the inner main belt.}
> In the next section we will discuss how V-type photometric candidates
336c338
< with the asteroid diameter, according to the figure legend.}  
---
> with the asteroid diameter, according to the figure legend.}
345,346c347,348
< We continue our analysis by studying the orbital region of 
< V-type photometric candidates in the outer main belt. We 
---
> We continue our analysis by studying the orbital region of
> V-type photometric candidates in the outer main belt. We
348,349c350,351
< test particles {\bf using the integrational set-up described in Carruba 
< et al. (2014b)}. 
---
> test particles  \textbf{using the integrator set-up described in Carruba
> et al. (2014b)}.
354,355c356,357
< a range between 2.825 and 3.278 AU in $a$, and $0^{\circ}$ and $24.0^{\circ}$ 
< in $i$, respectively.}.  The initial 
---
> a range between 2.825 and 3.278 AU in $a$, and $0^{\circ}$ and $24.0^{\circ}$
> in $i$, respectively.}.  The initial
358,360c360,362
< and a possible source of V-type asteroids.  
< We then computed synthetic proper elements $(a, e, sin(i))$ 
< and frequencies $(n,g,s)$ of these test particles with the approach 
---
> and a possible source of V-type asteroids.
> We then computed synthetic proper elements $(a, e, sin(i))$
> and frequencies $(n,g,s)$ of these test particles with the approach
369,373c371,375
< Black dots identify the orbital position in the plane of proper 
< $(a, sin(i))$ of each simulated test particle.  Color circles are 
< associated with asteroids likely to be in $z_1$ secular resonance 
< configurations. The other symbols have the same meaning as in 
< Fig.~\ref{fig:  V-type_external}.} 
---
> Black dots identify the orbital position in the plane of proper
> $(a, sin(i))$ of each simulated test particle.  Color circles are
> associated with asteroids likely to be in $z_1$ secular resonance
> configurations. The other symbols have the same meaning as in
> Fig.~\ref{fig:  V-type_external}.}
380c382
< appear as vertical bands with lesser density of test particles~\footnote{Of 
---
> appear as vertical bands with lesser density of test particles~\footnote{Of
382c384
< 14390  (1990 QP19), that is on the edge of the stable region near the 
---
> 14390  (1990 QP19), that is on the edge of the stable region near the
386c388
< panel B.  The main secular resonance in the outer main belt to appear in 
---
> panel B.  The main secular resonance in the outer main belt to appear in
388c390
< test particles whose combination of asteroidal secular frequencies 
---
> test particles whose combination of asteroidal secular frequencies
398c400
< Nevertheless, we studied the time dependence of the resonant argument of 
---
> Nevertheless, we studied the time dependence of the resonant argument of
400c402
< for the whole 37 V-type photometric candidates populations that we 
---
> for the whole 37 V-type photometric candidates populations that we
402c404
< the time-dependence of the resonant angles of the resonances $z_1, z_2, z_3, 
---
> the time-dependence of the resonant angles of the resonances $z_1, z_2, z_3,
406c408
< candidates in secular resonant states, 15 of which inside the 
---
> candidates in secular resonant states, 15 of which inside the
408,410c410,412
< found one object (85812 1998 WR22) inside the $3{\nu}_6-2{\nu}_5$ 
< resonance.  Three objects were in circulating orbits  
< close to the separatrix of the $z_1$ resonances, and three other 
---
> found one object (85812 1998 WR22) inside the $3{\nu}_6-2{\nu}_5$
> resonance.  Three objects were in circulating orbits
> close to the separatrix of the $z_1$ resonances, and three other
412,416c414,418
< resonance.  While past interactions with secular resonances may of 
< course not be excluded, overall secular dynamics seems to have 
< played a lesser role in the dynamical evolution of V-type 
< photometric candidates in the central main belt with respect 
< to the outer belt.  Further assessing the truth of this statement 
---
> resonance.  While past interactions with secular resonances may of
> course not be excluded, overall secular dynamics seems to have
> played a lesser role in the dynamical evolution of V-type
> photometric candidates in the central main belt with respect
> to the outer belt.  Further assessing the truth of this statement
418a421
> 
422,427c425,428
< To investigate the dynamical evolution of the 37 V-type candidates in the 
< outer main belt, we integrated clones of these objects with SWIFT-RMVSY, 
< the symplectic integrator of Bro\v{z} (1999) that simulates the 
< diurnal and seasonal versions of the Yarkovsky effect, {\bf using the 
< numerical set-up and values of Yarkovsky parameters discussed
< in (Carruba et al. (2014b).  As in that paper, we used the two sets 
---
> To investigate the dynamical evolution of the 37 V-type candidates in the
> outer main belt,  \textbf {we used the same methods and procedures presented in Carruba et al. (2014b).
>  We integrated clones of these objects with SWIFT-RMVSY,
> the symplectic integrator of Bro\v{z} (1999)}.  \sout{that simulates the diurnal and seasonal versions of the Yarkovsky effect,  using the numerical set-up and values of Yarkovsky parameters discussed in Carruba et al. (2014b).}       \textbf {As in that paper, we used the two sets
429,437c430,440
< the orbital plane that maximize the velocity of the drift caused by 
< the Yarkovsky effect, and did not considered re-orientations.}
< 
< As in Carruba et al. (2014b), we first performed “fast simulations” of 
< these asteroids, assuming that all objects had 100 m diameters.  Objects 
< so small will drift much faster than the real asteroids, allowing for 
< quicker simulations time-scales. On the other end, details of evolution 
< in higher order mean-motion and secular resonances may be lost because 
< of the faster drift.  We therefore also performed simulations 
---
> the orbital plane that maximize the velocity of the drift caused by
> the Yarkovsky effect, and did not considered re-orientations. To further investigate the dynamical evolution of V-type candidates in the outer main belt, we performed 'fast'  and 'slow' numerical simulations of these asteroids, assuming that all asteroids had 100 m diameters. Our results are presented in Figs 5 and 6,  which
> refer to the final orbital evolution on the  $a-sin(i)$ plane of V-type photometric candidates in the region of Eos, Koronis and Magnya.
> }
> 
> \sout{As in Carruba et al. (2014b), we first performed “fast simulations” of
> these asteroids, assuming that all objects had 100 m diameters.  Objects
> so small will drift much faster than the real asteroids, allowing for
> quicker simulations time-scales. On the other end, details of evolution
> in higher order mean-motion and secular resonances may be lost because
> of the faster drift.  We therefore also performed simulations
439,441c442,444
< factors $cos (30^\circ)$ and $cos (60◦^\circ)$ to account for values of 
< the spin obliquity other than zero, that we will discuss later on 
< in this section.
---
> factors $cos (30^\circ)$ and $cos (60◦^\circ)$ to account for values of
> the spin obliquity other than zero, that we will discuss later on
> in this section.}
446,458c449,462
< We obtained synthetic proper elements every 1.2 Myr for all 
< the simulated asteroids, with the approach described in Knezevic 
< and Milani (2003), modified as described in Carruba (2010), over 200 Myr.  In 
< Fig.~\ref{fig: yarko} we show the dynamical paths of clones of 
< particles in the Dembowska region (panel A), Eos (panel B) and 
< Magnya (panel C) in the $(a,sin(i))$ plane.  
< Blue dots represent snaphsots of the orbital 
< evolution of clones of real asteroids with $0◦^\circ$ obliquity, while 
< yellow dots are associated with clones with $180◦^\circ$ obliquity.  
< 
< In the Koronis region there were eight photometric candidates.  
< Four of them were not able to cross 
< the 7J:-3A mean-motion  resonance, including the (10537) V-type confirmed
---
> We obtained synthetic proper elements every 1.2 Myr for all
> the simulated asteroids, with the approach used in Carruba et al. (2014b) \sout{described in Knezevic
> and Milani (2003), modified as described in Carruba (2010)}, over 200 Myr.  In
> Fig.~\ref{fig: yarko} we show the dynamical paths of clones of
> particles in the Dembowska region (panel A), Eos (panel B) and
> Magnya (panel C) in the $(a,sin(i))$ plane.
> Blue dots represent snaphsots of the orbital
> evolution of clones of real asteroids with $0◦^\circ$ obliquity, while
> yellow dots are associated with clones with $180◦^\circ$ obliquity.
> 
> In the Koronis region there were eight photometric candidates.
> Four of them were not able to cross
> the 7J:-3A mean-motion
> resonance, including the (10537) V-type confirmed
461,464c465,471
< In panel B we observe the orbital evolution of 19 asteroids  in the Eos
< region: only 3 of them were not able to cross the 7J:-3A mean-motion 
< resonance,  and all clones were able to cross the 
< 9J:-4A and  3J:-5S:-3A mean-motion resonances, 
---
> In panel B we observe the orbital evolution of 19 asteroids
>  in the Eos
> region: only 3 of them were not able to cross the 7J:-3A mean-motion
> resonance,
>  and all clones were able to cross the
> 9J:-4A and
> 3J:-5S:-3A mean-motion resonances,
467c474
< in the Magnya region.  Three objects were not able to cross the 
---
> in the Magnya region.  Three objects were not able to cross the
470,474c477,481
< and the ${\nu}_6$ secular resonance.  Overall, we found one particle 
< that managed to cross the main dynamical 
< barrier of the 5J:-2A resonance and none that crossed the  
< 2J:-1A mean motion resonance, suggesting that comunication 
< between the central and outer main belt might be possible, but not likely 
---
> and the ${\nu}_6$ secular resonance.  Overall, we found one particle
> that managed to cross the main dynamical
> barrier of the 5J:-2A resonance and none that crossed the
> 2J:-1A mean motion resonance, suggesting that comunication
> between the central and outer main belt might be possible, but not likely
485c492
<    
---
> 
489c496
<    
---
> 
493c500
< \caption{Orbital evolution of 100 m clones of V-type photometric 
---
> \caption{Orbital evolution of 100 m clones of V-type photometric
500,501c507,508
< Finally, we also observed minor changes of inclination caused by 
< secular resonances (mostly by the $z_1$ resonance) 
---
>  \textbf{We also verified that} minor changes of inclination caused by
> secular resonances (mostly by the $z_1$ resonance)
505,507c512,514
< the Koronis and Magnya regions may be possible, but that passing 
< from the Eos to the Magnya region and vice-versa might a more unlikely 
< event.  We will further investigate this hypothesis in the next subsection. 
---
> the Koronis and Magnya regions may be possible, but that passing
> from the Eos to the Magnya region and vice-versa might a more unlikely
> event.  We will further investigate this hypothesis in the next subsection.
512,528c519,529
< To further investigate the dynamical evolution of V-type candidates 
< in the outer main belt, we {\bf also performed “slow” simulations of clones of 
< the same particles studied in Sect~\ref{sec: yarko_fast}. We took 
< the WISE values of the diameters for the test particles for 
< which such information was available}, and we used the methods 
< described in Sect~\ref{sec: V-type_groups} for the other particles.  
< We also took six values of spin obliquities, $0^\circ$ , $30^\circ$ , 
< $60^\circ$ , $120^\circ$ , $150^\circ$ , and $180^\circ$, in order to 
< sample different speeds of drifts caused by the Yarkovsky force.  
< We integrated our test particles over 1 Byr, with the 
< same integration scheme used in Sect~\ref{sec: yarko_fast}. 
< {\bf As in Carruba et al. (2014b), because of the longer integration 
< time used in these 
< runs, we computed proper elements every 4.9 Myr instead of 
< the 1.2 Myr used in Sect~\ref{sec: yarko_fast}.}
< 
< %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
---
> \textbf{In this simulations, we considered clones of the same particles studied in Sect~\ref{sec: yarko_fast}. We took
> the WISE values of the diameters for the test particles for
> which such information was available, and we used the methods
> described in Sect~\ref{sec: V-type_groups} for the other particles. In order to
> sample different speeds of drifts caused by the Yarkovsky force, we took values of spin obliquities in the range from $0^\circ$  to $180^\circ$. The values initially assumed were $0^\circ$, $30^\circ$, $60^\circ$, $120^\circ$, $150^\circ$, and $180^\circ$.
> All simulations were numerically integrated for 1 Byr, with the
> same integration scheme used in Sect~\ref{sec: yarko_fast}.
>  As in Carruba et al. (2014b), because of the longer integration
> time used in these
> runs, we computed proper elements every 4.9 Myr.}
> %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
533c534,535
<    \end{minipage}%  
---
>    \end{minipage}%
> 
535d536
<    
538,539c539,540
<    \end{minipage}%   
<    
---
>    \end{minipage}%
> 
543,544c544,545
< \caption{Orbital evolution of clones of real asteroids in the region 
< of Koronis, Eos, and Magnya, integrated over 1 Byr.  
---
> \caption{Orbital evolution of clones of real asteroids in the region
> of Koronis, Eos, and Magnya, integrated over 1 Byr.
549c550
< %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  
---
> %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
555,558c556,559
< in the Eos region, and  with obliquities of $60^{\circ}$ and $150^{\circ}$ in 
< the Magnya region (panels A, B, and C, respectively).   Prograde clones 
< elements are shown as blue dots, 
< retrograde clones ones are identified as yellow dots.  Other symbols 
---
> in the Eos region, and  with obliquities of $60^{\circ}$ and $150^{\circ}$ in
> the Magnya region (panels A, B, and C, respectively).   Prograde clones
> elements are shown as blue dots,
> retrograde clones ones are identified as yellow dots.  Other symbols
560c561
< for other values of the obliquities, and will not be shown for the sake 
---
> for other values of the obliquities, and will not be shown for the sake
563,567c564,568
< Of the 222 integrated clones, none was able to go from the Koronis 
< region to the Eos and Magnya areas or to cross the 7J:-3A mean-motion 
< resonance.  Only 2 particles from the Eos region managed to cross the 
< 7J:-3A mean-motion resonance and go into the Koronis area, i.e., 1.8\% 
< of the total, suggesting that communication 
---
> Of the 222 integrated clones, none was able to go from the Koronis
> region to the Eos and Magnya areas or to cross the 7J:-3A mean-motion
> resonance.  Only 2 particles from the Eos region managed to cross the
> 7J:-3A mean-motion resonance and go into the Koronis area, i.e., 1.8\%
> of the total, suggesting that communication
570,576c571,577
< More difficult to interpret were the results near the boundaries of the 
< Magnya and Eos region.   Of the 114 integrated clones in the Eos area, 
< 3 particles (2.7\%) managed to reach the Magnya area and survive 
< (mostly because of interaction with the $z_1$ secular resonance). 
< Conversely, of the 60 particles integrated in the Magnya region, 
< only 5 (4.5\%) were able to reach the Eos region via diffusion in 
< the $z_1$ secular resonance and interaction with other mean-motion 
---
> More difficult to interpret were the results near the boundaries of the
> Magnya and Eos region.   Of the 114 integrated clones in the Eos area,
> 3 particles (2.7\%) managed to reach the Magnya area and survive
> (mostly because of interaction with the $z_1$ secular resonance).
> Conversely, of the 60 particles integrated in the Magnya region,
> only 5 (4.5\%) were able to reach the Eos region via diffusion in
> the $z_1$ secular resonance and interaction with other mean-motion
578c579
< In all the six simulations, we only observed 3 particles that 
---
> In all the six simulations, we only observed 3 particles that
580,581c581,582
< resonance, but were not able to cross it.  (1459) Magnya is confined in a zone 
< defined by the $z_1$ and 2J:-1A resonances, and no particles managed 
---
> resonance, but were not able to cross it.  (1459) Magnya is confined in a zone
> defined by the $z_1$ and 2J:-1A resonances, and no particles managed
586,587c587,588
< regions.  While some mixing among V-type photometric candidates coming 
< from the Magnya and Eos parent body could be possible, our results still 
---
> regions.  While some mixing among V-type photometric candidates coming
> from the Magnya and Eos parent body could be possible, our results still
589c590
< of V-type photometric candidates in the outer main belt. 
---
> of V-type photometric candidates in the outer main belt.
595c596
< Carruba et al. (2014b) recently estimated the long term effect of 
---
> Carruba et al. (2014b) recently estimated the long term effect of
601,602c602,603
< zero mean, there will be a $1\sigma$ (= 68.27\%) probability that  
< the root mean square translation distance (or quadratic mean) after $n$ 
---
> zero mean, there will be a $1\sigma$ (= 68.27\%) probability that
> the root mean square translation distance (or quadratic mean) after $n$
607,610c608,611
< the possible arrival of differentiated bodies in the main belt, 
< the root mean square translation in $\sin(i)$ would be of 
< 0.0130. Considering our boundary between the inclination regions of Eos 
< and Magnya at $\sin(i) = 0.24$, there are only 2 Magnya objects 
---
> the possible arrival of differentiated bodies in the main belt,
> the root mean square translation in $\sin(i)$ would be of
> 0.0130. Considering our boundary between the inclination regions of Eos
> and Magnya at $\sin(i) = 0.24$, there are only 2 Magnya objects
614c615
< with massive asteroids may have furnished an additional mechanism 
---
> with massive asteroids may have furnished an additional mechanism
617c618
<   
---
> 
623,624c624,625
< of V-type photometric candidates in the the outer main belt. 
< For these purposes, we: 
---
> of V-type photometric candidates in the the outer main belt.
> For these purposes, we:
628c629
< \item Revised the current knowledge on confirmed 
---
> \item Revised the current knowledge on confirmed
631c632
< photometric candidates in the region for a total of 37 possible V-type 
---
> photometric candidates in the region for a total of 37 possible V-type
633c634
< of the Eos family, and statistical considerations suggest that Eos could be 
---
> of the Eos family, and statistical considerations suggest that Eos could be
639c640
< of the V-type photometric candidates and masses of these objects.   The 
---
> of the V-type photometric candidates and masses of these objects.   The
642c643
< Only 1.35\% of the mass escavated from the craters in Vesta is currently 
---
> Only 1.35\% of the mass escavated from the craters in Vesta is currently
650,651c651,652
< \item Studied the dynamical evolution of clones of V-type photometric 
< candidates in the area under the influence of Yarkovsky and YORP forces, 
---
> \item Studied the dynamical evolution of clones of V-type photometric
> candidates in the area under the influence of Yarkovsky and YORP forces,
655,658c656,659
< possibly associated with the parent bodies of (349) Dembowska, (221) 
< Eos, and (1459) Magnya.  While communication across the 7J:-3A mean-motion 
< resonance seems to be a rare event, up to $\simeq 20\%$ of bodies from the 
< Magnya region could have reached the Eos area.  Mixing between the Magnya 
---
> possibly associated with the parent bodies of (349) Dembowska, (221)
> Eos, and (1459) Magnya.  While communication across the 7J:-3A mean-motion
> resonance seems to be a rare event, up to $\simeq 20\%$ of bodies from the
> Magnya region could have reached the Eos area.  Mixing between the Magnya
660c661
< rule out a three source scenario.  
---
> rule out a three source scenario.
666,672c667,673
< photometric candidates in the outer main belt.  Contrary to the case of the 
< central main belt, mixing between different zones material may occur in 
< somewhat larger proportion (up to 5\%), but communication across the 
< 7J:-3A mean-motion resonance seems an unlikely event for km-sized asteroid. 
< A study of mineralogical properties of V-type photometric candidates in 
< the region could in principle provide further clues to the possible 
< origin of basaltic material in the outer main belt, and on our 
---
> photometric candidates in the outer main belt.  Contrary to the case of the
> central main belt, mixing between different zones material may occur in
> somewhat larger proportion (up to 5\%), but communication across the
> 7J:-3A mean-motion resonance seems an unlikely event for km-sized asteroid.
> A study of mineralogical properties of V-type photometric candidates in
> the region could in principle provide further clues to the possible
> origin of basaltic material in the outer main belt, and on our
679c680
< {\bf We thank an anonymous reviewer for comments and suggestions 
---
> {\bf We thank an anonymous reviewer for comments and suggestions
681c682
< We would like to thank the S\~{a}o Paulo State Science Foundation 
---
> We would like to thank the S\~{a}o Paulo State Science Foundation
684,690c685,691
< This publication makes use of data products from the Wide-field 
< Infrared Survey Explorer, which is a joint project of the University 
< of California, Los Angeles, and the Jet Propulsion Laboratory/California 
< Institute of Technology, funded by the National Aeronautics and Space 
< Administration.  This publication also makes use of data products 
< from NEOWISE, which is a project of the Jet Propulsion 
< Laboratory/California Institute of Technology, funded by the Planetary 
---
> This publication makes use of data products from the Wide-field
> Infrared Survey Explorer, which is a joint project of the University
> of California, Los Angeles, and the Jet Propulsion Laboratory/California
> Institute of Technology, funded by the National Aeronautics and Space
> Administration.  This publication also makes use of data products
> from NEOWISE, which is a project of the Jet Propulsion
> Laboratory/California Institute of Technology, funded by the Planetary
697,699c698,700
< Table~\ref{table: aster_V2} reports the asteroid identification, 
< its proper $a,e,$ and $sin(i)$, its absolute magnitude ($H$), 
< diameter ($D$), and geometric albedo ($p_V$), according to the WISE mission, 
---
> Table~\ref{table: aster_V2} reports the asteroid identification,
> its proper $a,e,$ and $sin(i)$, its absolute magnitude ($H$),
> diameter ($D$), and geometric albedo ($p_V$), according to the WISE mission,
703,705c704,706
< asteroids in the outer main belt, and diameters computed according 
< to {\bf Eq. 8 in Carruba et al. (2014)} (for simplicity, 
< we do not report these data in the Table). 
---
> asteroids in the outer main belt, and diameters computed according
> to \textbf{Eq. 8 in Carruba et al. (2014)} (for simplicity,
> we do not report these data in the Table).
709c710
< \caption{{\bf List of V-type photometric candidates in the 
---
> \caption{{\bf List of V-type photometric candidates in the
714c715
< \hline\toprule 
---
> \hline\toprule
720c721
< \hline 
---
> \hline
725c726
<    55613&   2.9143&     0.0250&     0.1397&    14.34&      	&       &\\    
---
>    55613&   2.9143&     0.0250&     0.1397&    14.34&      	&       &\\
727c728
<   141036&   2.9444&     0.0987&     0.0342&    15.78&      	&       &\\   
---
>   141036&   2.9444&     0.0987&     0.0342&    15.78&      	&       &\\
729c730
<    
---
> 
737c738
<    61877&   3.0607&     0.0700&     0.0302&    14.75&      	&       &\\   
---
>    61877&   3.0607&     0.0700&     0.0302&    14.75&      	&       &\\
740,742c741,743
<    97502&   3.0541&     0.2407&     0.1289&    14.43&     3.0460& 0.2751&\\ 
<   105041&   3.0403&     0.1583&     0.1847&    14.09&      	&       &\\ 
<   106205&   3.0776&     0.1163&     0.0381&    15.50&      	&       &\\  
---
>    97502&   3.0541&     0.2407&     0.1289&    14.43&     3.0460& 0.2751&\\
>   105041&   3.0403&     0.1583&     0.1847&    14.09&      	&       &\\
>   106205&   3.0776&     0.1163&     0.0381&    15.50&      	&       &\\
752c753
<  
---
> 
755c756
< \hline  
---
> \hline
775c776
< \bibitem[\protect\citeauthoryear{Bottke}{2006}]{bottke_2006} Bottke, W. F., 
---
> \bibitem[\protect\citeauthoryear{Bottke}{2006}]{bottke_2006} Bottke, W. F.,
782c783
< \bibitem[\protect\citeauthoryear{Carruba}{2010}]{Carruba_2010b} Carruba, V., 
---
> \bibitem[\protect\citeauthoryear{Carruba}{2010}]{Carruba_2010b} Carruba, V.,
785,786c786,787
< \bibitem[\protect\citeauthoryear{Carruba}{2014a}]{Carruba_2013} Carruba, 
< V., Domingos, R. C., Nesvorn\'{y}, D., Roig, F., Souami, D., 2014a, 
---
> \bibitem[\protect\citeauthoryear{Carruba}{2014a}]{Carruba_2013} Carruba,
> V., Domingos, R. C., Nesvorn\'{y}, D., Roig, F., Souami, D., 2014a,
789,790c790,791
< \bibitem[\protect\citeauthoryear{Carruba}{2014b}]{Carruba_2014b} Carruba, 
< V., M. E. Huaman, R. C. Domingos, C. R. Dos Santos, D. Souami 2014b, 
---
> \bibitem[\protect\citeauthoryear{Carruba}{2014b}]{Carruba_2014b} Carruba,
> V., M. E. Huaman, R. C. Domingos, C. R. Dos Santos, D. Souami 2014b,
796c797
< \bibitem[\protect\citeauthoryear{Demeo}{2013}]{DeMeo_2013} 
---
> \bibitem[\protect\citeauthoryear{Demeo}{2013}]{DeMeo_2013}
799,800c800,801
< \bibitem[\protect\citeauthoryear{DeSanctis}{2011}]{DeSanctis_2011} 
< De Sanctis, M.~C., Ammannito, E., Migliorini, A., et al.\ 2011a, 
---
> \bibitem[\protect\citeauthoryear{DeSanctis}{2011}]{DeSanctis_2011}
> De Sanctis, M.~C., Ammannito, E., Migliorini, A., et al.\ 2011a,
803,804c804,805
< \bibitem[\protect\citeauthoryear{DeSanctis}{2011b}]{2011epsc.conf..212D} de Sanctis, M.~C., 
< Migliorini, A., Luzia Jasmim, F., et al.\ 2011b, EPSC-DPS Joint Meeting 
---
> \bibitem[\protect\citeauthoryear{DeSanctis}{2011b}]{2011epsc.conf..212D} de Sanctis, M.~C.,
> Migliorini, A., Luzia Jasmim, F., et al.\ 2011b, EPSC-DPS Joint Meeting
808c809
< Duffard, R., \& Roig, F.\ 2009, P\&SS, 57, 229. 
---
> Duffard, R., \& Roig, F.\ 2009, P\&SS, 57, 229.
810c811
< \bibitem[\protect\citeauthoryear{farinella}{1998}]{farinella_1998} 
---
> \bibitem[\protect\citeauthoryear{farinella}{1998}]{farinella_1998}
814,815c815,816
< Giorgini, J. D., and 9 co-authors, Bulletim of the American 
< Astronomical Society 28, 1158, 
---
> Giorgini, J. D., and 9 co-authors, Bulletim of the American
> Astronomical Society 28, 1158,
818,820c819,821
< \bibitem[\protect\citeauthoryear{harris}{2002}]{Harris_2002} Harris, A. W., 
< Lagerros, J. S. V., 2002, Asteroids III, W. F. Bottke Jr., A. Cellino, P. 
< Paolicchi, and R. P. Binzel (eds), University of Arizona Press, Tucson, 
---
> \bibitem[\protect\citeauthoryear{harris}{2002}]{Harris_2002} Harris, A. W.,
> Lagerros, J. S. V., 2002, Asteroids III, W. F. Bottke Jr., A. Cellino, P.
> Paolicchi, and R. P. Binzel (eds), University of Arizona Press, Tucson,
823c824
< \bibitem[\protect\citeauthoryear{knezevic}{2003}]{knezevic_2003} 
---
> \bibitem[\protect\citeauthoryear{knezevic}{2003}]{knezevic_2003}
826c827
< \bibitem[\protect\citeauthoryear{lazzaro}{2000}]{lazzaro_2000} Lazzaro, D., 
---
> \bibitem[\protect\citeauthoryear{lazzaro}{2000}]{lazzaro_2000} Lazzaro, D.,
828c829
<  
---
> 
831,832c832,833
<  
< \bibitem[\protect\citeauthoryear{masiero}{2011}]{Masiero_2011} 
---
> 
> \bibitem[\protect\citeauthoryear{masiero}{2011}]{Masiero_2011}
835c836
< \bibitem[\protect\citeauthoryear{mainzer}{2011}]{Mainzer_2011} 
---
> \bibitem[\protect\citeauthoryear{mainzer}{2011}]{Mainzer_2011}
838c839
< \bibitem[\protect\citeauthoryear{machuca}{2011}]{Machuca_2012} Machuca, 
---
> \bibitem[\protect\citeauthoryear{machuca}{2011}]{Machuca_2012} Machuca,
841c842
< \bibitem[\protect\citeauthoryear{milani}{1994}]{milani_1994} Milani, A., 
---
> \bibitem[\protect\citeauthoryear{milani}{1994}]{milani_1994} Milani, A.,
844c845
< \bibitem[\protect\citeauthoryear{milani}{2013}]{milani_2013} Milani, A., 
---
> \bibitem[\protect\citeauthoryear{milani}{2013}]{milani_2013} Milani, A.,
847c848
< \bibitem[\protect\citeauthoryear{michtchenko}{2002}] Michtchenko, T.~A., 
---
> \bibitem[\protect\citeauthoryear{michtchenko}{2002}] Michtchenko, T.~A.,
850c851
< \bibitem[\protect\citeauthoryear{moskovitz}{2008}]{Moskovitz_2008} Moskovitz, 
---
> \bibitem[\protect\citeauthoryear{moskovitz}{2008}]{Moskovitz_2008} Moskovitz,
853,855c854,856
< \bibitem[\protect\citeauthoryear{Mothe-Diniz}{2008}]{2008Icar..195..277M} 
< Moth{\'e}-Diniz, T., Carvano, J.~M., Bus, S.~J., Duffard, R., 
< \& Burbine, T.~H.\ 2008, Icarus, 195, 277 
---
> \bibitem[\protect\citeauthoryear{Mothe-Diniz}{2008}]{2008Icar..195..277M}
> Moth{\'e}-Diniz, T., Carvano, J.~M., Bus, S.~J., Duffard, R.,
> \& Burbine, T.~H.\ 2008, Icarus, 195, 277
857c858
< \bibitem[\protect\citeauthoryear{wright}{2010}]{Wrigth_2010} 
---
> \bibitem[\protect\citeauthoryear{wright}{2010}]{Wrigth_2010}
860c861
< \bibitem[\protect\citeauthoryear{zappala}{1995}]{zappala_1995} Zappal\`{a}, 
---
> \bibitem[\protect\citeauthoryear{zappala}{1995}]{zappala_1995} Zappal\`{a},
862c863
< Icarus, 116, 291. 
---
> Icarus, 116, 291.

